Logical peering for interdomain networking on testbeds

Research testbed fabrics have potential to support long-lived, evolving, interdomain experiments, including opt-in application traffic across multiple campuses and edge sites. We propose abstractions and security infrastructure to facilitate multi-domain networking, and a reusable controller toolkit (ExoPlex) for network service providers (NSPs) running in testbed-hosted virtual network slices. We demonstrate the idea on the ExoGENI testbed, which allows slices to interconnect and exchange traffic over peering links by mutual consent. Each ExoPlex NSP runs a peering controller that manages its interactions with its linked peers and controls the NSP's dataplane network via SDN. Our approach expresses policies for secure peering and routing in a declarative language---logical peering. The prototype uses logic rules to verify IP prefix ownership, filter and validate route advertisements, and implement user-specified policies for connectivity and path control in networks with multiple transit NSPs.

==> data/result.tex <==
ain] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:08:43 [main] DEBUG e.s.c.e.ExoSdxManager - Flow table: NSP1 - e0
00:08:43 [main] DEBUG e.s.s.e.ExoSliceManager - [NSP1-129.7.98.24] run commands: sudo ovs-ofctl dump-flows br0
00:08:47 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x10000, duration=332.636s, table=0, n_packets=1, n_bytes=98, idle_age=216, priority=50,ip,nw_src=192.168.30.0/24,nw_dst=192.168.10.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:29:21,mod_dl_dst:fa:16:3e:00:4e:54,output:2
00:08:47 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x20000, duration=329.945s, table=0, n_packets=1, n_bytes=98, idle_age=4, priority=50,ip,nw_src=192.168.40.0/24,nw_dst=192.168.10.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:29:21,mod_dl_dst:fa:16:3e:00:4e:54,output:2
00:08:47 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x40000, duration=282.592s, table=0, n_packets=1, n_bytes=98, idle_age=216, priority=50,ip,nw_src=192.168.10.0/24,nw_dst=192.168.30.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:7b:8f,mod_dl_dst:fa:16:3e:00:60:47,output:1
00:08:47 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x50000, duration=267.929s, table=0, n_packets=1, n_bytes=98, idle_age=4, priority=50,ip,nw_src=192.168.10.0/24,nw_dst=192.168.40.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:7b:8f,mod_dl_dst:fa:16:3e:00:60:47,output:1
00:08:47 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:08:47 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:08:47 [main] DEBUG e.s.c.e.ExoSdxManager - Flow table: NSP1 - e1
00:08:47 [main] DEBUG e.s.s.e.ExoSliceManager - [NSP1-129.7.98.119] run commands: sudo ovs-ofctl dump-flows br0
00:08:53 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x10000, duration=337.314s, table=0, n_packets=1, n_bytes=98, idle_age=222, priority=50,ip,nw_src=192.168.30.0/24,nw_dst=192.168.10.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:60:47,mod_dl_dst:fa:16:3e:00:7b:8f,output:1
00:08:53 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x20000, duration=334.625s, table=0, n_packets=1, n_bytes=98, idle_age=9, priority=50,ip,nw_src=192.168.40.0/24,nw_dst=192.168.10.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:60:47,mod_dl_dst:fa:16:3e:00:7b:8f,output:1
00:08:53 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x40000, duration=288.427s, table=0, n_packets=1, n_bytes=98, idle_age=222, priority=50,ip,nw_src=192.168.10.0/24,nw_dst=192.168.30.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:6c:cf,mod_dl_dst:fa:16:3e:00:2b:b6,output:2
00:08:53 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x50000, duration=273.900s, table=0, n_packets=1, n_bytes=98, idle_age=9, priority=50,ip,nw_src=192.168.10.0/24,nw_dst=192.168.40.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:43:f4,mod_dl_dst:fa:16:3e:00:70:92,output:3
00:08:53 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:08:53 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:08:53 [main] DEBUG e.s.c.e.ExoSdxManager - Flow table: NSP2 - e1
00:08:53 [main] DEBUG e.s.s.e.ExoSliceManager - [NSP2-129.7.98.87] run commands: sudo ovs-ofctl dump-flows br0
00:08:58 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x10000, duration=331.307s, table=0, n_packets=1, n_bytes=98, idle_age=222, priority=50,ip,nw_src=192.168.40.0/24,nw_dst=192.168.20.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:77:1e,mod_dl_dst:fa:16:3e:00:33:b3,output:1
00:08:58 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x30000, duration=285.040s, table=0, n_packets=1, n_bytes=98, idle_age=222, priority=50,ip,nw_src=192.168.20.0/24,nw_dst=192.168.40.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:35:a3,mod_dl_dst:fa:16:3e:00:1a:96,output:2
00:08:58 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:08:58 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:08:58 [main] DEBUG e.s.c.e.ExoSdxManager - Flow table: NSP2 - e0
00:08:58 [main] DEBUG e.s.s.e.ExoSliceManager - [NSP2-129.7.98.91] run commands: sudo ovs-ofctl dump-flows br0
00:09:02 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x10000, duration=336.386s, table=0, n_packets=1, n_bytes=98, idle_age=227, priority=50,ip,nw_src=192.168.40.0/24,nw_dst=192.168.20.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:65:0b,mod_dl_dst:fa:16:3e:00:77:06,output:2
00:09:02 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x30000, duration=288.949s, table=0, n_packets=1, n_bytes=98, idle_age=227, priority=50,ip,nw_src=192.168.20.0/24,nw_dst=192.168.40.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:33:b3,mod_dl_dst:fa:16:3e:00:77:1e,output:1
00:09:02 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:09:02 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:09:02 [main] DEBUG e.s.c.e.ExoSdxManager - Flow table: NSP3 - e0
00:09:03 [main] DEBUG e.s.s.e.ExoSliceManager - [NSP3-129.7.98.46] run commands: sudo ovs-ofctl dump-flows br0
00:09:08 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x10000, duration=346.488s, table=0, n_packets=1, n_bytes=98, idle_age=237, priority=50,ip,nw_src=192.168.30.0/24,nw_dst=192.168.10.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:2b:b6,mod_dl_dst:fa:16:3e:00:6c:cf,output:2
00:09:08 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x30000, duration=318.213s, table=0, n_packets=1, n_bytes=98, idle_age=237, priority=50,ip,nw_src=192.168.10.0/24,nw_dst=192.168.30.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:52:48,mod_dl_dst:fa:16:3e:00:73:6a,output:1
00:09:08 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:09:08 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:09:08 [main] DEBUG e.s.c.e.ExoSdxManager - Flow table: NSP3 - e1
00:09:08 [main] DEBUG e.s.s.e.ExoSliceManager - [NSP3-129.7.98.30] run commands: sudo ovs-ofctl dump-flows br0
00:09:12 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x10000, duration=350.445s, table=0, n_packets=1, n_bytes=98, idle_age=241, priority=50,ip,nw_src=192.168.30.0/24,nw_dst=192.168.10.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:73:6a,mod_dl_dst:fa:16:3e:00:52:48,output:1
00:09:12 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x30000, duration=323.351s, table=0, n_packets=1, n_bytes=98, idle_age=241, priority=50,ip,nw_src=192.168.10.0/24,nw_dst=192.168.30.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:13:02,mod_dl_dst:fa:16:3e:00:7e:72,output:2
00:09:12 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:09:12 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:09:12 [main] DEBUG e.s.c.e.ExoSdxManager - Flow table: SDX1 - e1
00:09:12 [main] DEBUG e.s.s.e.ExoSliceManager - [SDX1-129.7.98.69] run commands: sudo ovs-ofctl dump-flows br0
00:09:18 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x10000, duration=368.815s, table=0, n_packets=1, n_bytes=98, idle_age=247, priority=50,ip,nw_src=192.168.30.0/24,nw_dst=192.168.10.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:30:34,mod_dl_dst:fa:16:3e:00:16:51,output:1
00:09:18 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x20000, duration=366.219s, table=0, n_packets=1, n_bytes=98, idle_age=34, priority=50,ip,nw_src=192.168.40.0/24,nw_dst=192.168.10.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:30:34,mod_dl_dst:fa:16:3e:00:16:51,output:1
00:09:18 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x30000, duration=355.836s, table=0, n_packets=1, n_bytes=98, idle_age=242, priority=50,ip,nw_src=192.168.40.0/24,nw_dst=192.168.20.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:30:34,mod_dl_dst:fa:16:3e:00:16:51,output:1
00:09:18 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x40000, duration=305.835s, table=0, n_packets=1, n_bytes=98, idle_age=247, priority=50,ip,nw_src=192.168.10.0/24,nw_dst=192.168.30.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:4e:54,mod_dl_dst:fa:16:3e:00:29:21,output:2
00:09:18 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x50000, duration=298.039s, table=0, n_packets=1, n_bytes=98, idle_age=242, priority=50,ip,nw_src=192.168.20.0/24,nw_dst=192.168.40.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:77:06,mod_dl_dst:fa:16:3e:00:65:0b,output:3
00:09:18 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x60000, duration=292.432s, table=0, n_packets=1, n_bytes=98, idle_age=34, priority=50,ip,nw_src=192.168.10.0/24,nw_dst=192.168.40.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:4e:54,mod_dl_dst:fa:16:3e:00:29:21,output:2
00:09:18 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:09:18 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:09:18 [main] DEBUG e.s.c.e.ExoSdxManager - Flow table: SDX1 - e0
00:09:18 [main] DEBUG e.s.s.e.ExoSliceManager - [SDX1-128.194.6.139] run commands: sudo ovs-ofctl dump-flows br0
00:09:22 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x10000, duration=374.128s, table=0, n_packets=1, n_bytes=98, idle_age=251, priority=50,ip,nw_src=192.168.30.0/24,nw_dst=192.168.10.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:1f:6f,mod_dl_dst:fa:16:3e:00:22:6d,output:3
00:09:22 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x20000, duration=371.525s, table=0, n_packets=1, n_bytes=98, idle_age=39, priority=50,ip,nw_src=192.168.40.0/24,nw_dst=192.168.10.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:1f:6f,mod_dl_dst:fa:16:3e:00:22:6d,output:3
00:09:22 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x30000, duration=361.150s, table=0, n_packets=1, n_bytes=98, idle_age=247, priority=50,ip,nw_src=192.168.40.0/24,nw_dst=192.168.20.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:34:65,mod_dl_dst:fa:16:3e:00:51:92,output:2
00:09:22 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x40000, duration=309.940s, table=0, n_packets=1, n_bytes=98, idle_age=252, priority=50,ip,nw_src=192.168.10.0/24,nw_dst=192.168.30.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:16:51,mod_dl_dst:fa:16:3e:00:30:34,output:1
00:09:22 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x50000, duration=301.983s, table=0, n_packets=1, n_bytes=98, idle_age=247, priority=50,ip,nw_src=192.168.20.0/24,nw_dst=192.168.40.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:16:51,mod_dl_dst:fa:16:3e:00:30:34,output:1
00:09:22 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x60000, duration=296.389s, table=0, n_packets=1, n_bytes=98, idle_age=39, priority=50,ip,nw_src=192.168.10.0/24,nw_dst=192.168.40.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:16:51,mod_dl_dst:fa:16:3e:00:30:34,output:1
00:09:22 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:09:22 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:09:22 [main] DEBUG e.s.c.e.ExoSdxManager - Flow table: NSP4 - e0
00:09:22 [main] DEBUG e.s.s.e.ExoSliceManager - [NSP4-129.7.98.113] run commands: sudo ovs-ofctl dump-flows br0
00:09:27 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x10000, duration=364.754s, table=0, n_packets=1, n_bytes=98, idle_age=44, priority=50,ip,nw_src=192.168.40.0/24,nw_dst=192.168.10.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:70:92,mod_dl_dst:fa:16:3e:00:43:f4,output:3
00:09:27 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x20000, duration=356.122s, table=0, n_packets=1, n_bytes=98, idle_age=251, priority=50,ip,nw_src=192.168.40.0/24,nw_dst=192.168.20.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:1a:96,mod_dl_dst:fa:16:3e:00:35:a3,output:2
00:09:27 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x40000, duration=318.996s, table=0, n_packets=1, n_bytes=98, idle_age=251, priority=50,ip,nw_src=192.168.20.0/24,nw_dst=192.168.40.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:14:f7,mod_dl_dst:fa:16:3e:00:74:bf,output:1
00:09:27 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x50000, duration=316.312s, table=0, n_packets=1, n_bytes=98, idle_age=44, priority=50,ip,nw_src=192.168.10.0/24,nw_dst=192.168.40.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:14:f7,mod_dl_dst:fa:16:3e:00:74:bf,output:1
00:09:27 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:09:27 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:09:27 [main] DEBUG e.s.c.e.ExoSdxManager - Flow table: NSP4 - e1
00:09:27 [main] DEBUG e.s.s.e.ExoSliceManager - [NSP4-129.7.98.120] run commands: sudo ovs-ofctl dump-flows br0
00:09:35 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x10000, duration=371.818s, table=0, n_packets=1, n_bytes=98, idle_age=51, priority=50,ip,nw_src=192.168.40.0/24,nw_dst=192.168.10.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:74:bf,mod_dl_dst:fa:16:3e:00:14:f7,output:1
00:09:35 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x20000, duration=363.175s, table=0, n_packets=1, n_bytes=98, idle_age=259, priority=50,ip,nw_src=192.168.40.0/24,nw_dst=192.168.20.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:74:bf,mod_dl_dst:fa:16:3e:00:14:f7,output:1
00:09:35 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x40000, duration=327.254s, table=0, n_packets=1, n_bytes=98, idle_age=259, priority=50,ip,nw_src=192.168.20.0/24,nw_dst=192.168.40.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:e5:5f,mod_dl_dst:fa:16:3e:00:32:aa,output:2
00:09:35 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x50000, duration=324.533s, table=0, n_packets=1, n_bytes=98, idle_age=51, priority=50,ip,nw_src=192.168.10.0/24,nw_dst=192.168.40.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:e5:5f,mod_dl_dst:fa:16:3e:00:32:aa,output:2
00:09:35 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:09:35 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:09:35 [main] DEBUG e.s.c.e.ExoSdxManager - Flow table: SDX2 - e1
00:09:35 [main] DEBUG e.s.s.e.ExoSliceManager - [SDX2-128.227.10.111] run commands: sudo ovs-ofctl dump-flows br0
00:09:39 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x10000, duration=371.151s, table=0, n_packets=1, n_bytes=98, idle_age=268, priority=50,ip,nw_src=192.168.30.0/24,nw_dst=192.168.10.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:18:ce,mod_dl_dst:fa:16:3e:00:2a:78,output:1
00:09:39 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x20000, duration=370.043s, table=0, n_packets=1, n_bytes=98, idle_age=56, priority=50,ip,nw_src=192.168.40.0/24,nw_dst=192.168.10.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:18:ce,mod_dl_dst:fa:16:3e:00:2a:78,output:1
00:09:39 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x30000, duration=357.569s, table=0, n_packets=1, n_bytes=98, idle_age=268, priority=50,ip,nw_src=192.168.10.0/24,nw_dst=192.168.30.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:7b:a0,mod_dl_dst:fa:16:3e:00:5e:09,output:3
00:09:39 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x40000, duration=355.133s, table=0, n_packets=1, n_bytes=98, idle_age=264, priority=50,ip,nw_src=192.168.40.0/24,nw_dst=192.168.20.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:18:ce,mod_dl_dst:fa:16:3e:00:2a:78,output:1
00:09:39 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x50000, duration=337.602s, table=0, n_packets=1, n_bytes=98, idle_age=264, priority=50,ip,nw_src=192.168.20.0/24,nw_dst=192.168.40.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:7c:4b,mod_dl_dst:fa:16:3e:00:36:af,output:2
00:09:39 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x60000, duration=334.886s, table=0, n_packets=1, n_bytes=98, idle_age=56, priority=50,ip,nw_src=192.168.10.0/24,nw_dst=192.168.40.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:7c:4b,mod_dl_dst:fa:16:3e:00:36:af,output:2
00:09:39 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:09:39 [main] DEBUG e.s.c.e.ExoSdxManager - ------------------
00:09:39 [main] DEBUG e.s.c.e.ExoSdxManager - Flow table: SDX2 - e0
00:09:39 [main] DEBUG e.s.s.e.ExoSliceManager - [SDX2-129.7.98.117] run commands: sudo ovs-ofctl dump-flows br0
00:09:44 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x10000, duration=376.403s, table=0, n_packets=1, n_bytes=98, idle_age=273, priority=50,ip,nw_src=192.168.30.0/24,nw_dst=192.168.10.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:7e:72,mod_dl_dst:fa:16:3e:00:13:02,output:3
00:09:44 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x20000, duration=375.288s, table=0, n_packets=1, n_bytes=98, idle_age=61, priority=50,ip,nw_src=192.168.40.0/24,nw_dst=192.168.10.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:32:aa,mod_dl_dst:fa:16:3e:00:e5:5f,output:2
00:09:44 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x30000, duration=361.466s, table=0, n_packets=1, n_bytes=98, idle_age=273, priority=50,ip,nw_src=192.168.10.0/24,nw_dst=192.168.30.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:2a:78,mod_dl_dst:fa:16:3e:00:18:ce,output:1
00:09:44 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x40000, duration=360.376s, table=0, n_packets=1, n_bytes=98, idle_age=268, priority=50,ip,nw_src=192.168.40.0/24,nw_dst=192.168.20.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:32:aa,mod_dl_dst:fa:16:3e:00:e5:5f,output:2
00:09:44 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x50000, duration=341.596s, table=0, n_packets=1, n_bytes=98, idle_age=268, priority=50,ip,nw_src=192.168.20.0/24,nw_dst=192.168.40.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:2a:78,mod_dl_dst:fa:16:3e:00:18:ce,output:1
00:09:44 [main] DEBUG e.s.c.e.ExoSdxManager -  cookie=0x60000, duration=338.908s, table=0, n_packets=1, n_bytes=98, idle_age=61, priority=50,ip,nw_src=192.168.10.0/24,nw_dst=192.168.40.0/24 actions=dec_ttl,mod_dl_src:fa:16:3e:00:2a:78,mod_dl_dst:fa:16:3e:00:18:ce,output:1

==> sections/Questions.tex <==
SAFE routing:
1. Can't detect or prevent spoofing, packet alteration, or packet replay from any trusted AS?
2. How the destination or the source verify that its policies are enforced? 
The destination can check the ingress filtering chain of upstream ASes.
3. Can we attest installed ingress filtering rules?
4. Path is valid unless two trusted ASes on the path collude to redirect the traffic, i.e. 



OPT: 
1. source authentication Overhead?
2. waste in bandwidth for carrying those headers (20\%)
3. Require changes in routers

Passport:  The source AS stamps the packet at its border. Can't protect against spoofing attacks from within the source AS.



==> sections/connectivity.tex <==
  

==> sections/related.tex <==
{\bf Logical trust.}  Trust/authorization logic~\cite{abadi93:accesscalculus,lampson92:authentication,spki-rfc2693,jim:sd3:2001,Li02:RT,detreville:binder:2002,Sendlog:Abadi:2007,abadi08, Schneider:2011:NAL:1952982.1952990} is a unifying formalism that can capture these attribute-based mechanisms and policies declaratively and concisely, minimizing the need for custom software, formats, and protocols to implement each design choice.  
The contributions of this paper (and of SAFE) are orthogonal to the details of SAFE's trust logic, which prefers Datalog with a standard syntax to balance expressive power, tractability, and accessibility for practical use.   In fact, Datalog-with-says is provably the most expressive tractable logic for trust: other logics are either less powerful and lack essential features (SPKI/SDSI~\cite{spki-rfc2693,abac-spki}, RT0~\cite{Li02:RT}), or are merely syntactic variants of Datalog, or else are intractable and are therefore (in our view) not suited to practical use.

Grid-inspired research has yielded several PKI-based trust systems that are logical in that they
combine roles and delegations with some
form of declarative policy~\cite{gt4-abac}.  Examples include the PERMIS~\cite{permis02,permis-modular08} system used in European grid initiatives.  These systems generally follow the approach pioneered by SPKI/SDSI, but they introduce custom policy languages.    Most recently, FLANC has been proposed as a custom logic for software-defined network exchanges (SDX)~\cite{Gupta:2016:FLANC}, but it is no more powerful than Datalog with constraints~\cite{Li03:constraint}, or else it is intractable.


{\bf XACML.}  Some cloud federation work proposes use of the XACML access control standard, which is now common in industry.  It is now understood that XACML is a subset of Datalog.  In contrast to XACML, Datalog-with-says has a rigorous formal semantics, so policies are verifiable.  It also extends assertions and policy rules with attribution ({\bf says}); this feature enables reasoning from authenticated policy rules and assertions gathered from multiple sources, which is crucial in federated scenarios.

==> sections/reviews.tex <==
====== Workshop Reviews 1 =======
> *** Weaknesses: What are the major reasons NOT to accept the paper? [Be brief.]

Paper is dense to read with many assumptions and concepts background that are not properly presented. The significance of the work can be improved with some application use case (e.g., video or science data workflow). Also, the implementation and experimentation is tied to ExoGENI testbed, and more information is needed for others to repeat the implementation/experiments.

A general discussion can be included on how one without access to the ExoGENI testbed can attempt to recreate and test proposed approaches.

There is a statement that performance and scale of experiments are bounded by the current limitations of ExoGENI. However, more justification can be provided for the values and parameters chosen in the experiments. For example, why is the maximum route length chosen to be 10? What are the considerations for choosing a certain number of NSPs in a simulation as well as in practical settings?

A separate background and working of the SAFE engine should be provided for making the paper more self-contained and readable.

A discussion on the factors that cause overheads with proposed approach should be presented, along with best practices to minimize the overheads.

======= Workshop Reviews 2 =======

> *** Weaknesses: What are the major reasons NOT to accept the paper? [Be brief.]

There is some confusion, as mentioned above, as to the paper's relationship to testbeds. I am convinced of the need for better security abstractions for interdomain routing. I am convinced that testbeds that span multiple domains need a security architecture. I am less convinced that the authors have demonstrated that they have provided what, itself, could be a "testbed for trust".

> *** Detailed Comments: Please provide detailed comments that will help the TPC assess the paper and help provide feedback to the authors.

If the authors really want to make the case that they are providing a "testbed for trust", I think they need to show how experimenters would not simply be testing various aspects of the system described here, ExoPlex, but would be testing ideas that are truly general.

I think the paper stands even without the "testbed for trust" claim, however, as an example of a good use of a testbed.

======= Workshop Reviews 3 =======
> *** Weaknesses: What are the major reasons NOT to accept the paper? [Be brief.]

It would be useful to see the security policies expressed in datalog, and see more clearly how those get implemented in the controller by showing the rules installed (there is a little of this in Fig. 3) but more would be nice.

I know, the paper covers a lot of ground...

> *** Detailed Comments: Please provide detailed comments that will help the TPC assess the paper and help provide feedback to the authors.

Although this paper has a focus on the security policies you've implemented, I feel it needs an example of the datalog logical trust language so we can see how that gets translated into code at the controller and then into rules in a switch? 

How do you know that your datalog is consistent with other policies?  What if policies conflict?  There is no dicussion about how these are resolved.

In IV, I guess the "customer networks" are A-D?

Why did you omit NSP 3 and 4 from your Experiment 1?

In IV.C why did you use synthetic topologies and random peering?  So I guess this part was not run in ExoGENI?

Fig. 4, y-axis label should be "Authorization Throughput"?


==> sections/spoof.tex <==
\ifdefined\DEBUG
{\color{red} Note: Anti-Spoofing and Path Validation are only compiled in double-column version}

{\bf Anti-spoofing} {\color{red} We should also talk about threat models} Volunteering ingress filtering on periphery routers~\cite{bcp38} are light-weight but less effective, as spoofed traffic can still be injected from networks without appropriate ingress filter or compromised networks.
Dataplane approaches include Passport~\cite{yang2008passport}, ICING~\cite{Naous11:icing} and OPT~\cite{opt2014lightweight}.  These solutions require the source host (or AS) to stamp each packet with one Message Authentication Code (MAC) for each AS (or router) on the path to the destination. At each hop, a router extracts its MAC from the packet header and verifies it using a secret key shared with the sender.  Dataplane approaches offer strong source authentication and path validation, but they increase packet sizes, introduce validation overhead for each packet at each hop, and must generate and manage the shared keys by some method. Moreover, firewalls may block packets with extra header fields. 

Combining routing path control and ingress filtering between ASes, we can prevent traffic spoofing from untrusted networks. Our approach works in the control plane and requires neither packet verification in the dataplane nor upgrades to routers. 

ExoPlex augments secure routing with anti-spoofing  
The source and destination can protect their traffic from passing through untrusted ASes with path control policies. 
To avoid spoofing, the source and destination trust an AS only if it meets the following two requirements. First, no one can spoof traffic (packet injection) from within its network. Only the valid owner of the IP prefix can send traffic from the source IP address. Second, the AS implements such ingress filter at the edges such that traffic are allowed only if the neighbor AS is authorized by both source and destination's path control policies.
 
{\bf Path validation} OPT~\cite{opt2014lightweight} adds an Origin and Path Verification (OPV) field in the packet header that allows path validation by each hop on the path and the destination. Every hop on the path compute the hash with the previous OFV value and the key shared with source and destination and update the field. 

We argue that we can also validate the path with route choice verification and stronger ingress filtering. Each AS on the path makes certified statements about their choices of next hop for traffic with specific prefix pair. An AS is a authenticated carrier for traffic with specific prefix pair if it is compliant to both source and destination path control policies, and is stated by the upstream AS as the next hop for the prefix pair. Each trusted AS on the path implements ingress filtering that only traffic from authenticated upstream AS are allowed ({\color{red}stronger requirements than anti-spoofing requirements}). 

The certified statements about next-hop choices are also linked to allow end-to-end verification. Here is an example. For the path $<A, NSP_1, NSP_2, B>$, let's consider how B verifies the path. A posts a statement that $NSP_1$ is the next hop for traffic from A to B $(prefix A, prefix B)$, and notifies $NSP_1$ via their peering channel. Then $NSP_1$ posts a statement that $NSP_2$ is the next hop, linking to A's statement showing that NSP1 itself is authenticated. And $NSP_1$ notifies $NSP_2$ about the choice. $NSP_2$ verifies that $NSP_1$ is authenticated and white list traffic with the prefix pair from $NSP_1$. With stronger ingress filtering, we can make sure that traffic can only go through the path that is stated hop-by-hop, unless two trusted AS on the path collude to deviate the path. For example, if $NSP_1$ states $NSP_2$ as the next hop for$(prefix A, prefix B)$, it cannot send the traffic to any other trusted AS as it won't be allowed by ingress filtering of other trusted ASes. 
\fi

==> slog/ingress-policy.tex <==
allowIngress(?UpstreamAS, ?SrcPrefix, ?DstPrefix) :-
    validCarrier(?UpstreamAS, ?AggSrcPrefix, ?AggDstPrefix),
    ?SrcPrefix <: ?AggSrcPrefix,
    ?DstPrefix <: ?AggDstPrefix.
    %?UpstreamAS: nextHop(\$Self, ?SrcPrefix, ?DstPrefix). 
  
validCarrier(?AS, ?SrcPrefix, ?DstPrefix) :-
    ?UpstreamAS: nextHop(?AS, ?SrcPrefix, ?DstPrefix),
    validCarrier(?UpstreamAS, ?AggSrcPrefix, ?AggDstPrefix),
    ?SrcPrefix <: ?AggSrcPrefix,
    ?DstPrefix <: ?AggDstPrefix.
    
    
validCarrier(?AS, ?SrcPrefix, "0.0.0.0/0"):- 
    ownPrefix(?AS, ?SrcPrefix).
    
% The upstream AS tells downstream AS a list of prefix pairs for which the upsteam AS chooses the downstream AS as next hop. The upstream AS also passes tokens to safe sets that prove itself a valid carrier for those prefix pairs.
% Each AS can split the prefix pair and set different next hops for different parts. For example, the source chooses AS1 as next hop for all traffic from its prefix, <SrcPrefix, "0.0.0.0/0">, and AS1 chooses different next hops for different destinations. 
% When implementing routing and ingress filtering rules in dataplane, the ASes can aggregate prefixes owned by different principals. But in logic statements, they can't aggregate such information. For example, AS1 chooses AS2 as next hop for traffic from "10.0.0.0/24" (owned by Alice) and "10.0.1.0/24" (owned by bob). AS1 can install a flow that matches on "10.0.0.0/23" to route the  traffic to AS2.
%However, in SAFE logic statement, AS1 can't say nextHop(AS2, "10.0.0.0/23", DstIP). It requires the logic engine to be able to aggregate range values to be able to verify such statement, which SAFE (or other known logic engine) doesn't support.

==> slog/safe-routing.tex <==
verifyRoute(?Owner,?DstIP,?Path) :-
  authorizedRoute(?Owner,?DstIPSet,?Path, $Self),
  ?DstIP <: ?DstIPSet.

authorizedRoute(?Owner,?DstIP,?Path,?AS):-
  eq([?Owner|?Tail],?Path),
  eq(?Tail,[]),
  ?Owner: advertise(?DstIP,?Path,?AS),
  ownPrefix(?Owner,?DstIP).

authorizedRoute(?Owner,?DstIP,?Path,?AS):-
  eq([?Head|?Tail],?Path),
  ?Head:advertise(?DstIP,?Path,?AS),
  ?Owner: authorizedAS(?Head, ?DstIP),
  authorizedRoute(?Owner,?IPSet,?Tail,?Head),
  ?DstIP <: ?IPSet.
